Do Input Gradients Highlight Discriminative Features?

Post-hoc gradient-based interpretability methods [Simonyan et al., 2013, Smilkov et al., 2017] that provide instance-specific explanations of model predictions are often based on assumption (A): magnitude of input gradients -- gradients of logits with respect to input -- noisily highlight discriminative task-relevant features. In this work, we test the validity of assumption (A) using a three-pronged approach. First, we develop an evaluation framework, DiffROAR, to test assumption (A) on four image classification benchmarks. Our results suggest that (i) input gradients of standard models (i.e., trained on original data) may grossly violate (A), whereas (ii) input gradients of adversarially robust models satisfy (A). Second, we introduce BlockMNIST, an MNIST-based semi-real dataset, that by design encodes a priori knowledge of discriminative features. Our analysis on BlockMNIST leverages this information to validate as well as characterize differences between input gradient attributions of standard and robust models. Finally, we theoretically prove that our empirical findings hold on a simplified version of the BlockMNIST dataset. Specifically, we prove that input gradients of standard one-hidden-layer MLPs trained on this dataset do not highlight instance-specific signal coordinates, thus grossly violating assumption (A). Our findings motivate the need to formalize and test common assumptions in interpretability in a falsifiable manner [Leavitt and Morcos, 2020]. We believe that the DiffROAR evaluation framework and BlockMNIST-based datasets can serve as sanity checks to audit instance-specific interpretability methods; code and data available at https://github.com/harshays/inputgradients.

==> checklist.tex <==
\section*{Checklist}

%%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please see~\Cref{sec:conc}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Please see~\Cref{app:theory} and~\Cref{app:conj}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Please see~\Cref{sec:real} and~\Cref{appendix:real}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See~\Cref{appendix:real}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See~\Cref{fig:real}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See~\Cref{appendix:real}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Please see~\Cref{sec:real}}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Code, trained models, and \semirealname~dataset will be open-sourced}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> oldreal.tex <==
%\section{Experiments on Real Data}
% Image Classification Tasks}
\harshay{todo, will finish this section today (thurs)}
In this section, we use~\evalname~to test whether input gradient attributions of standard and adversarially robust MLPs and CNNs trained on four image classification benchmarks satisfy or violate assumption~\premise.

In this section, we use our evaluation framework to analyze the gradient attribution quality, $\FHf(\AG, \cdot)$, in image classification tasks.
We first summarize our experiment setup and then outline key empirical findings.

\textbf{Datasets}: We consider two benchmark image classification datasets: \cifar~and \imnet. The \cifar~dataset~\cite{krizhevsky2009learning} comprises $60,000$ images in $10$ semantic classes. The \imnet~dataset is an open-sourced\footnote{\url{https://github.com/MadryLab/robustness/}} variant of Imagenet~\cite{imagenet_cvpr09}, in which $80,000$ images are grouped into $10$ high-level super-classes. \imnet~ enables us to work with Imagenet data without the computational overload of training models on the $1000$-way ILSVRC classification task ~\cite{ILSVRC15}. 

\textbf{Training Procedure}: We use ResNet18 and ResNet50~\cite{He2015} on \imnet~and \cifar~ datasets respectively. Unless mentioned otherwise, we use stochastic gradient descent (SGD) as the default optimizer, with momentum $0.9$, batch size $256$, $\ell_2$ regularization $0.0005$ and initial learning rate $0.1$ that decays by a factor of $0.75$ every $20$ epochs. Additionally, we use standard data augmentation, train models for at most $500$ epochs and stop early if train loss goes below $0.01$. In~\Cref{appendix:real}, we show that our empirical findings are robust to the choice of model architecture and SGD hyperparameters.



\textbf{Estimating Attribution Quality}: 
We estimate the attribution quality $\FHf(\AG,k)$ on real data as follows.
\vspace{-5px}
\begin{itemize}[leftmargin=*]
	\item Train a model on original training data to compute its input gradients $\mathcal{G}$ and its feature attribution scheme $\AG$.
	\item Given $\AG$ and fraction of unmasked pixels $k$, extract top-$k$ \& bottom-$k$ feature highlight schemes: $\At{k}$ \& $\Ab{k}$.
	\item Obtain top-$k$ train \& test data by \emph{unmasking only those} pixels in every image $x$ that are highlighted by attributions $\At{k}(x)$. Compute bottom-$k$ train \& test data using $\Ab{k}$.
	\item To estimate $\pred{\At{k}}$, \emph{retrain a new model} on top-$k$ unmasked train data and evaluate its accuracy on top-$k$ test data; analogously estimate $\pred{\Ab{k}}$ to obtain $\FHf(\AG, k)$.
\end{itemize}  
\vspace{-5px}
Also, note that (a) we average $\FHf(\AG, k)$ over $3$ runs for all models and values of level $k$, (b) use ResNet18 to retrain in in both tasks, and (c) unmask individual image pixels \emph{without} grouping them channel-wise. 

%	\item  For every image $x$, compute masked images---\emph{only unmask} pixels in images that are using top-$k$ and bottom-$k$ attributions respectively.

%First, we train a model $\mathcal{M}$ on the original dataset $D^{\text{train}}$ to compute its input gradients $\mathcal{G}$ and its feature attribution scheme $\AG$. 
%Then, given the fraction of unmasked pixels $k$, we extract $\At{k}$ and $\Ab{k}$, the top-$k$ and bottom-$k$ feature highlight schemes, and compute train and test datasets that comprise images masked using the top-$k$ and bottom-$k$ attributions.
%Next, to compute $\pred{\Ab{k}}$ and $\pred{\At{k}}$, we (i) apply the highlight scheme on images to obtain masked datasets, $(D^{\text{train}}_{A}, D^{\text{test}}_{\text{bot}})$, (ii) \emph{retrain} a new ResNet18 model usi

%Next, to compute $\pred{A}$, we apply $\At_k$ and $\Ab_k$ to images to obtain two sets of gradient-masked train and test datasets: $D^{\text{top}}$ and $D$

%Given model and k, we can compute attribution quality in M steps.
%First, we compute the input gradients scheme top bottom and obtain new datasets
%then, we use a resnet18 model on D to compute the predictive power and hence FH 
%Our results are averaged over three runs for evry model and hoice of k
%Also note that each pixel is treated separately and not grouped channel-wies

\begin{figure*}[t]
	\centering
	\includegraphics[width=\linewidth]{imgs/neurips21_real}
	\vspace{-15px}
	\caption{\hs{todo} 
	\FIG and \RFGI in benchmark image classification tasks. 
	The left and right subplots evaluate the quality $\FHf(\AG,k)$ of gradient-based attribution scheme $\AG$ of standard and adversarially robust models trained on \cifar and \imnet~respectively. 
	For standard models, when the fraction of unmasked pixels $k < 20\%$, input gradients exhibit \FIG, as $\FHf(\AG, k) < 0$. 
	That is, input coordinates that have the largest gradient magnitude are not as important performance-wise as the coordinates with smallest gradient magnitude.
	Conversely, $\{\ell_2,\ell_{\infty}\}$-adversarially trained models exhibit \RFGI as $\FHf(\AG,k) \geq 0$ for all $k$; input gradients fix \FIG and satisfy \premise~by highlighting relevant features over irrelevant features.} 
%	Additionally, note that (i) our results hold for $\ell_2$ and $\ell_{\infty}$ adversarial robustness and (ii) increasing the adversarial perturbation norm $\epsilon$ can improve attribution quality $\FHf(\AG, k)$. 
 \label{fig:real}
 \vspace{-5px}
\end{figure*}


\textbf{Experiment Results}: Figure~\ref{fig:real} illustrates the gradient attribution quality $\FHf(\AG,k)$ of standard and $\{\ell_2, \ell_{\infty}\}$-robust models trained on \cifar~and \imnet~data for level $k \in \{0.05, ..., 1.0\}$. We make the following observations:

\textbf{Feature Inversion in Gradients (\FIG)}: Standard ResNet18 and ResNet50 models trained on \cifar~and \imnet~exhibit \FIG. The shaded area in~\Cref{fig:real} illustrates that when level $k<20\%$, attribution quality $\FHf(\AG,k)$ is consistently negative. As discussed in~\Cref{sec:prelim}, this indicates that input gradients of standard models violate premise \premise, as the features with \emph{lowest} gradient magnitude have more predictive power of the labels than the features with \emph{highest} gradient magnitude. In other words, contrary to conventional wisdom, input gradients highlight irrelevant features and suppress relevant features in benchmark image classification tasks.

\textbf{Adversarial Robustness fixes \FIG (\RFGI)}:  
	As shown in~\Cref{fig:real}, for all $k$, adversarially trained models exhibit input gradients with consistently \emph{positive} attribution quality $\FHf(\AG, k)$.
	That is, models that are adversarially trained using $\ell_2$ or $\ell_{\infty}$ perturbations fix feature inversion in gradients (\FIG) on both datasets.
	Moreover, compared to standard models, adversarially trained models starkly highlight relevant features over irrelevant features.
	For example, on \imnet~, when $k=0.05$ (i.e., only $5\%$ of pixels unmasked), the attribution quality of $\ell_{\infty}$-robust model ($\epsilon=2/255$) and standard model equals $0.15$ and $-0.05$ respectively.
	We also observe that increasing the adversarial perturbation norm $\epsilon$ can significantly improve attribution quality $\FHf(\AG, .)$ for all $k$. 
	For instance, on \cifar~data, the attribution quality of $\l_{2}$-robust models trained with $\epsilon=0.50$ is consistently greater than than with $\ell_2=0.25$.
	To summarize, adversarial training not only mitigates \FIG but also improves the extent to which input gradient attributions \emph{separate} relevant features from irrelevant features.
	
\hs{appendix para mention that results continue to hold for large-scale CNNs but not FCNs -- that it's unreliable}
	
%	the gradient attribution quality of standard and $\ell_{\infty}$-robust model (\epsilon=8/255) 
%	
%	when $k=0.05$, $\ell_{\infty}$-robust ResNet50 trained on \cifar~with $\epsilon=8/255$ exhibits a $23\%$ gap in the predictive power of features corresponding to the top $5\%$ and bottom $5\%$ of gradient magnitude.
%
% trained on both datasets with multiple perturbation norm $\epsilon$, 
% 
%In other words, input gradients of robust models highlight relevant features over irrelevant features
%
% For adversarially trained models, $FHf(\AG,k) > 0$ for all values of $k$ showing that adversarially trained models do not suffer from \FI. Note that both $\textrm{Linf}$ and $\textrm{L2}$ robustness helps in fixing \FI.
%
%\textbf{Adversarial Robustness improves Attribution Quality}: Comparing the plots of $\textrm{L2}-0.50$ and $\textrm{L2}-0.25$ for \cifar~and $\textrm{Linf}-2$ and $\textrm{Linf}-1$ for \imnet, we see that models that are more robust are more resistant to \FI.




==> oldsetting.tex <==
\section{Preliminaries and Evaluation Metrics}
\label{sec:prelim}
In this section, we introduce our evaluation framework to measure the extent to which instance-specific explanations, or feature attributions, highlight relevant features over irrelevant features.
%In this section, we present our framework for evaluating  attribution schemes for highlighting task relevant features. 
%In next section, we will use this framework to evaluate the input gradients of standard and adversarially trained models for highlighting task relevant features.
We consider the standard classification setting, where we are given training data  $(x^{(i)},y^{(i)})$, for $i\in [n] \defeq \set{1,\cdots,n}$. 
Each data point $(x^{(i)},y^{(i)})$, where $x^{(i)} \in \R^d$ and $y^{(i)} \in \Y$ for some label set $\Y$, is drawn independently from a distribution $\D$ on $\R^d \times \Y$. 
For $j \in [d]$, $x^{(i)}_j$ denotes the $j^{\textrm{th}}$ coordinate of $x^{(i)}$. 
We refer to the $d$ coordinates of input $x^{(i)}$ as \emph{coordinates} or \emph{features} interchangeably. 
For a given $S \subseteq [d]$, the \emph{unmasking} operation retains the features in $S$ and zeros out those in $[d]\setminus S$, as defined below:

\begin{definition}[Unmasking]
	\label{def:unmask}
	Given a data point $x$ and a set $S \subseteq [d]$ of features, we define the \emph{unmasked} point $x^S$ as $x^S_j=x_j$ if $j \in S$ and $0$ if $j \notin S$.
\end{definition}

A \emph{feature highlight} scheme $A: \R^d\rightarrow \set{S: S\subseteq [d]}$ is a function that maps point $x$ to a subset $A(x) \subseteq[d]$ of features.
To put it in context, given feature highlight scheme $A$, point $x^{A(x)}$ denotes the unmasked version of point $x$, such that $x^{A(x)}_j = x_j$ if and only if $j \in A(x)$.
We can measure the \emph{predictive power} of a feature highlight scheme $A$, on a given model class $\M$ such as ResNets, as the best classification accuracy that can be attained by $\M$ \emph{exclusively using instance-specific features highlighted by $A$}:

\begin{definition}[Predictive power]
	\label{def:predpower}
	Given a feature highlight scheme $A$, and a model class $\M$, its predictive power is defined as:
	\begin{align*}
		\pred{A} \defeq \sup_{f \in \M, f: \R^d \rightarrow \Y} \ED{\ind{f(x^{A(x)})=y}}.
	\end{align*}
\end{definition}

\textbf{Estimating $\pred{A}$}: 
In practice, it is not possible to provably and efficiently optimize over all functions $f\in \M$, so we estimate $\pred{A}$ in two steps. 
First, using highlight scheme $A$, we generate $A$-unmasked data of the form $\displaystyle\set{\left(\left(x^{(i)}\right)^{A(x^{(i)})},y^{(i)}\right): i \in [n]}$ that are unmasked using highlight scheme $A$.
	Then, we train a new classifier of model class $\M$ on $A$-unmasked train data and evaluate its accuracy on $A$-unmasked held-out data. In our experiments on \cifar~and \imnet~in Section~\ref{sec:real}, we take the model class to be ResNets. Appendix~\ref{appendix:real} shows that our results continue to hold for other model classes such as VGG~\cite{simonyan2014very}.
Note that our approach to estimate $\pred{A}$ shares commonalities with the retraining framework~\cite{Hooker2019ABF} discussed in~\Cref{sec:related}.
%
%training a new classifier on \emph{unmasked} training data $\set{\left(\left(x^{(i)}\right)^{A(x^{(i)})},y^{(i)}\right): i \in [n]}$ and computing its accuracy on \emph{unmasked} held-out data. \harshay{need to emphasize that both train and test are unmasked using $A$ to evaluate $\pred{A}$, not clear right now.}

More generally, A \emph{feature attribution} scheme $\A: \R^d \rightarrow \set{\sigma: \sigma \mbox{ is a permutation of } [d]}$
%\footnote{Note the overload of notation between \emph{feature highlight} scheme and \emph{feature attribution} scheme. The usage however will be clear from context.}
maps an input data point $x$ to a permutation, or ordering, $\A(x): [d] \rightarrow [d]$ of the features. 
%\harshay{we use coordinates here but ``features'' to define $A$.}
The {feature attribution} scheme $\A$ and level $k\leq d$ induce two natural \emph{feature highlight} schemes $\At{k}$ and $\Ab{k}$ that highlight the $k$ top-most and bottom-most attributions respectively. In other words,
\begin{align*}
\At{k}(x) &\defeq \set{\A(x)_{j}: j \leq k}, \\
\Ab{k}(x) &\defeq \set{\A(x)_{j}: d-k < j \leq d}.
\end{align*}

\textbf{Evaluating Attribution Quality}: 
Attribution schemes $\A$ that satisfy premise \premise~must place (i) relevant features, which are important for classification, at the top of the attribution order and (ii) irrelevant features at the bottom.
%One expectation from an attribution scheme is that features important for classification are placed in the top of the permutation, while the irrelevant features are placed in the bottom of the permutation. 
To formalize this notion, we relate the quality of an attribution scheme $\A$ at level $k$ to the difference between the predictive power of $\At{k}$ and $\Ab{k}$, the two natural feature highlight schemes defined above. The quality of attribution scheme $\A$ is formally defined below:
\begin{align*}
	\FHf(\A,k) = \pred{\At{k}} - \pred{\Ab{k}}.
\end{align*}
The \emph{sign} of the attribution quality $\FHf(\A, \cdot)$ indicates whether the attribution scheme $\A$ highlights relevant features over irrelevant features.
%satisfies or violates premise \premise. 
If $\FHf(\A, \cdot) < 0$, the predictive power of highlight scheme $\At{k}$, which comprises top-most attributions, is \emph{less} than that of $\Ab{k}$.
In other words, when $\FHf(\A, \cdot) < 0$, $\A$ suppresses relevant features and highlights irrelevant features, and vice-versa. 
%Conversely, when $\FHf(\A, \cdot) > 0$, $\A$ highlights relevant features and suppresses irrelevant features.
%thereby satisfying \premise.

The \emph{magnitude} of the attribution quality $\FHf(\A, \cdot)$ quantifies the extent to which the ordering in attribution scheme $\A$ separates relevant features from irrelevant features.
Consider a \emph{random} feature attribution $\A$, where $\A(x)$ is chosen uniformly at random from all orderings of $[d]$.
In this case, $\mathbb{E}[\FHf(\A,k)]=0$ because the highlight schemes $\At{k}$ and $\Ab{k}$ have identical distributions for every level $k$.
In other words, the attribution equality $\FHf(\A, \cdot)$ is zero when $\A$ neither highlights nor suppresses relevant features.

%For a given highlight scheme $\A$, positive (resp. negative) values of $\FHf(\A,\cdot)$ indicate that $\A$ highlights (resp. suppresses) task relevant features over task irrelevant features. Similarly, the magnitude of $\FHf(\A,\cdot)$ indicates the extent of this highlighting or suppression (resp. $\FHf(\A,\cdot)$ is greater than or less than $0$). In comparison, a random feature attribution $\A$, where $\A(x)$ is chosen uniformly from among all permutations of $[d]$ leads to identical distributions for $\At{k}$ and $\Ab{k}$ and hence leads to $\mathbb{E}[\FHf(\A,k)]=0$ for every $k$, capturing the fact that the ordering of features given by $\A$ neither highlights nor suppresses task relevant features over task irrelevant features.



\textbf{Gradient-based Attributions}: Given a neural network parameterized by $\theta$ and data point $x$, denote the  model prediction by $\hat{y}(\theta,x)$ and loss (e.g., cross-entropy) on $(x, y)$ by $\L(\theta,(x,y))$. 
	Recall that $\A(x)$ is a permutation over $[d]$ for every $x \in \R^d$. 
	A \emph{gradient-based attribution scheme} $\AG$ is induced by the magnitude of the input gradient: $\nabla_x \L(\theta,(x,\hat{y}(\theta,x))$\footnote{Note that we differentiate only with respect to the input and not the $x$ appearing inside $\hat{y}(\theta,x)$}. In particular, if the $j^{th}$ entry in the input gradient has the $i^{th}$ largest \emph{magnitude}, then $\AG(x)_i=j$. 
	
	While our evaluation framework is general enough for any feature attribution scheme $\A$, we focus on {gradient-based attributions} for two reasons. 
	First, well-known attribution methods are heavily based on gradients. For instance, SmoothGrad~\cite{smilkov2017smoothgrad} computes input gradients of randomly perturbed data points, and Integrated Gradients~\cite{sundararajan2017axiomatic} compute input gradients of linearly-interpolated data points.
	Second, as discussed in~\Cref{sec:related}, unlike input gradients, well-known attribution methods fail multiple sanity checks~\cite{adebayo2018sanity,kindermans2019reliability}, thereby clearly lacking fidelity.
	Additionally, the quality of gradient-based attribution schemes, $\FHf(\AG, \cdot)$, also indicates whether $\AG$ satisfies or violates the premise \premise. For example, when $\FHf(\AG, \cdot) < 0$, $\AG$ violates \premise~by highlighting irrelevant features over relevant features.

%Note that we consider \emph{instance-specific}, or \emph{local}, attribution schemes, which depend on the given instance, as opposed to \emph{global} schemes, which provide the same highlights/attributions for all instances~\cite{}. 
% COMMENT: perhaps better addressed in introduction rather than here.
% \harshay{confirm what global means in attribution context and cite}


